Simulate to Generalize: Scaling Stateful Supervision for API-calling Agents using LLM World Models

Training agents that generalize to unseen, stateful environments requires a massive dataset of state-changing trajectories covering a vast and diverse set of APIs. However, scaling this broad supervision is severely bottlenecked by the immense effort required to implement and populate fully-executable environments across a broad spectrum of domains. To bypass this barrier, we introduce a data generation pipeline that decouples data synthesis from environment construction by leveraging LLMs as digital world models. Starting from only a list of broad domain names, our automated pipeline synthesizes diverse APIs and tasks. To produce trajectories, a teacher agent iteratively solves these tasks while an LLM simulator dynamically tracks state and provides coherent API responses on-the-fly. Finally, an automated judge filters the trajectories for quality. Fine-tuning on our broad synthetic dataset yields significant performance gains on AppWorld and OfficeBench, two challenging stateful benchmarks featuring environments completely unseen during training. These results establish our LLM world model-based synthesis approach as a highly scalable path for training generalizable, stateful API-calling agents.

==> sections/0_abstract.tex <==
\begin{abstract}
Training agents that generalize to unseen, stateful environments requires a massive dataset of state-changing trajectories covering a vast and diverse set of APIs. However, scaling this broad supervision is severely bottlenecked by the immense effort required to implement and populate fully-executable environments across a broad spectrum of domains. To bypass this barrier, we introduce a data generation pipeline that decouples data synthesis from environment construction by leveraging LLMs as digital world models. Starting from only a list of broad domain names, our automated pipeline synthesizes diverse APIs and tasks. To produce trajectories, a teacher agent iteratively solves these tasks while an LLM simulator dynamically tracks state and provides coherent API responses on-the-fly. Finally, an automated judge filters the trajectories for quality. Fine-tuning on our broad synthetic dataset yields significant performance gains on AppWorld and OfficeBench, two challenging stateful benchmarks featuring environments completely unseen during training. These results establish our LLM world model-based synthesis approach as a highly scalable path for training generalizable, stateful API-calling agents.

\end{abstract}



%Training API-calling agents capable of generalizing to unseen, stateful applications requires a massive dataset of interactive trajectories featuring state-changing actions across a vast and diverse set of APIs. Traditionally, collecting such data mandates implementing executable environments and populating them with rich and interconnected underlying states. While building a small stateful environment for a few target applications is manageable, scaling this infrastructure and data curation to a broad spectrum of applications creates a severe bottleneck. To overcome this scaling barrier, we introduce a synthetic data generation approach that leverages LLMs as digital world models to dynamically synthesize agentic trajectories, allowing us to scale up broad supervision with minimal human intervention. Starting with only a list of broad domain names, our fully automated pipeline first synthesizes a diverse set of stateful applications, their corresponding API specifications, and complex tasks solvable using these APIs. To generate trajectories, a teacher agent iteratively solves each task while an LLM simulator—acting as an on-the-fly digital world model—provides coherent API responses conditioned on the task context and interaction history. Finally, an automated judge filters the trajectories for quality. Our experiments demonstrate that fine-tuning on this synthetic dataset yields significant performance gains on AppWorld and OfficeBench, two challenging stateful benchmarks featuring applications disjoint from our training data. These results establish our LLM world model-based synthesis approach as a highly scalable path for training stateful API-calling agents that robustly generalize to unseen APIs and environments.
